Racial Disparities in Pulse Oximetry Cannot Be Fixed With Race-Based Correction

Studies have shown pulse oximeter measurements of blood oxygenation have statistical bias that is a function of race, which results in higher rates of occult hypoxemia, i.e., missed detection of dangerously low oxygenation, in patients of color. This paper further characterizes the statistical distribution of pulse ox measurements, showing they also have a higher variance for patients racialized as Black, compared to those racialized as white. We show that no single race-based correction factor will provide equal performance in the detection of hypoxemia. The results have implications for racially equitable pulse oximetry.

==> header.tex <==
\newcommand{\dd}[1]{{\tfrac{\partial}{\partial #1}}}
\newcommand{\dfd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dtwod}[1]{\frac{\partial^2}{\partial #1^2}}
\newcommand{\dtwodd}[2]{\frac{\partial^2}{\partial #1 \partial #2}}
\newcommand{\dndd}[3]{\frac{\partial^{#3}}{\partial {#1} \cdots \partial {#2}}}
\newcommand{\dtwofdd}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\Var}[2]{\mbox{Var}_{#1}\left[ {#2} \right]}
\newcommand{\Cov}[1]{\mbox{Cov}\left( {#1} \right)}
\newcommand{\E}[2]{E_{#1}\left[ {#2} \right]}
\newcommand{\I}[1]{\mathrm{I}_{#1}}
\newcommand{\PR}[1]{P\left[{#1}\right]}
\newcommand{\RE}[1]{\mathbb{R} \left[{#1}\right]}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}
%\newcommand{\RE}{1}{{\mathbb{Re}\left\{{#1}\right\}}}
\newcommand{\argmin}[1]{\mathop{\mbox{argmin}}_{#1}}
\newcommand{\argmax}[1]{\mathop{\mbox{argmax}}_{#1}}
\newcommand{\argminX}{\argmin{ X: \; X^TX=I_D}}
\newcommand{\Order}[1]{\mathcal{O}\left( {#1} \right)}
\newcommand{\ds}[1]{\mathrm{d}{#1}}
\newcommand{\dv}[1]{\mathrm{d}\Vc{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\me}{\mathrm{e}}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\mI}{\mathbb{I}}
\newcommand{\vone}{\Vc{1}}
\newcommand{\vzero}{\Vc{0}}
\newcommand{\vI}{\Vc{I}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\diag}[1]{{\mbox{diag}\left\{{#1}\right\}}}
\newcommand{\bb}[0]{\bar{b}}
\newcommand{\bs}[0]{\bar{\sigma}}
\newcommand{\mbA}[0]{\mathbf{A}}
\newcommand{\mbB}[0]{\mathbf{B}}
\newcommand{\mbC}[0]{\mathbf{C}}
\newcommand{\mbD}[0]{\mathbf{D}}
\newcommand{\mbE}[0]{\mathbf{E}}
\newcommand{\mbF}[0]{\mathbf{F}}
\newcommand{\mbG}[0]{\mathbf{G}}
\newcommand{\mbH}[0]{\mathbf{H}}
\newcommand{\mbI}[0]{\mathbf{I}}
\newcommand{\mbJ}[0]{\mathbf{J}}
\newcommand{\mbK}[0]{\mathbf{K}}
\newcommand{\mbL}[0]{\mathbf{L}}
\newcommand{\mbM}[0]{\mathbf{M}}
\newcommand{\mbN}[0]{\mathbf{N}}
\newcommand{\mbO}[0]{\mathbf{O}}
\newcommand{\mbP}[0]{\mathbf{P}}
\newcommand{\mbQ}[0]{\mathbf{Q}}
\newcommand{\mbR}[0]{\mathbf{R}}
\newcommand{\mbS}[0]{\mathbf{S}}
\newcommand{\mbT}[0]{\mathbf{T}}
\newcommand{\mbU}[0]{\mathbf{U}}
\newcommand{\mbV}[0]{\mathbf{V}}
\newcommand{\mbW}[0]{\mathbf{W}}
\newcommand{\mbX}[0]{\mathbf{X}}
\newcommand{\mbY}[0]{\mathbf{Y}}
\newcommand{\mbZ}[0]{\mathbf{Z}}
\newcommand{\mba}[0]{\mathbf{a}}
\newcommand{\mbb}[0]{\mathbf{b}}
\newcommand{\mbc}[0]{\mathbf{c}}
\newcommand{\mbd}[0]{\mathbf{d}}
\newcommand{\mbe}[0]{\mathbf{e}}
\newcommand{\mbf}[0]{\mathbf{f}}
\newcommand{\mbg}[0]{\mathbf{g}}
\newcommand{\mbh}[0]{\mathbf{h}}
\newcommand{\mbi}[0]{\mathbf{i}}
\newcommand{\mbj}[0]{\mathbf{j}}
\newcommand{\mbk}[0]{\mathbf{k}}
\newcommand{\mbl}[0]{\mathbf{l}}
\newcommand{\mbm}[0]{\mathbf{m}}
\newcommand{\mbn}[0]{\mathbf{n}}
\newcommand{\mbo}[0]{\mathbf{o}}
\newcommand{\mbp}[0]{\mathbf{p}}
\newcommand{\mbq}[0]{\mathbf{q}}
\newcommand{\mbr}[0]{\mathbf{r}}
\newcommand{\mbs}[0]{\mathbf{s}}
\newcommand{\mbt}[0]{\mathbf{t}}
\newcommand{\mbu}[0]{\mathbf{u}}
\newcommand{\mbv}[0]{\mathbf{v}}
\newcommand{\mbtv}[0]{\mathbf{\tilde{v}}}
\newcommand{\mbw}[0]{\mathbf{w}}
\newcommand{\mbx}[0]{\mathbf{x}}
\newcommand{\mby}[0]{\mathbf{y}}
\newcommand{\mbty}[0]{\mathbf{\tilde{y}}}
\newcommand{\mbz}[0]{\mathbf{z}}
\newcommand{\mbzero}[0]{\mathbf{0}}
\newcommand{\mbalpha}[0]{{\boldsymbol{\alpha}}}
\newcommand{\mbdelta}[0]{{\boldsymbol{\delta}}}
\newcommand{\mbepsilon}[0]{{\boldsymbol{\epsilon}}}
\newcommand{\mbmu}[0]{{\boldsymbol{\mu}}}
\newcommand{\mbPi}[0]{{\boldsymbol{\Pi}}}
\newcommand{\mbpi}[0]{{\boldsymbol{\pi}}}
\newcommand{\mbtheta}[0]{{\boldsymbol{\theta}}}
\newcommand{\mbphi}[0]{{\boldsymbol{\phi}}}


\newcommand{\Definition}[2]{\vspace{0.1in} \noindent    {\begin{minipage}{\linewidth}\underline{\bf Def'n:}  {\it #1}\\
#2\end{minipage}}\vspace{0.1in} \\ }
\newcommand{\Lemma}[2]{\vspace{0.1in}\\ \noindent  {\begin{minipage}{\linewidth}\underline{\bf Lemma:}  {#1}\\
{\bf Proof:} #2 \end{minipage}}\vspace{0.1in} \\ }
\newcommand{\Theorem}[2]{\vspace{0.1in} \noindent \begin{minipage}{\linewidth}\underline{\bf Theorem:}
{#1} \\ {\bf Proof:} {#2} \end{minipage}\vspace{0.1in} \\ }
\newcommand{\StartOf}[1]{{\noindent \rule{\linewidth}{1pt}\\ \noindent \large \bf #1}\\}
\newcommand{\Today}[1]{{\noindent \large Today: #1}\\}
\newcommand{\Example}[1]{{\vspace{0.15in} \noindent \bf Example: #1}\\}
\newcommand{\Note}[1]{{\vspace{0.05in} \noindent {\bf Note:} #1}\\}
\newcommand{\IF}[1]{\,\,\,\, \mbox{if} \,\,\, #1}
\newcommand{\pdfarray}[2]{{ \left\{\begin{array}{ll} {#1}, & {#2} \\ 0, & o.w. \end{array}\right. }}
\newcommand{\pdfarrays}[4]{{ \left\{\begin{array}{ll} {#1}, & {#2} \\ {#3}, & {#4} \\ 0, & o.w. \end{array}\right. }}
\newcommand{\twooptions}[4]{{ \left\{\begin{array}{ll} {#1}, & {#2} \\ {#3}, & {#4} \end{array}\right. }}
\newcommand{\threeoptions}[6]{{ \left\{\begin{array}{ll} {#1}, & {#2} \\ {#3}, & {#4} \\ {#5}, & {#6} \end{array}\right. }}
\newcommand{\CDFarrays}[4]{{ \left\{\begin{array}{ll}
   0,    & {#3} < {#2} \\
   {#1}, & {#2} \le {#3} < {#4} \\
   1, & {#3} \ge {#4} \end{array}\right. }}
\newcommand{\CDFarray}[3]{{ \left\{\begin{array}{ll}
   0,    & {#3} < {#2} \\
   {#1}, & {#3} \ge {#2} \end{array}\right. }}
\newcommand{\CCDFarrays}[4]{{ \left\{\begin{array}{ll}
   1,    & {#3} < {#2} \\
   {#1}, & {#2} \le {#3} < {#4} \\
   0, & {#3} \ge {#4} \end{array}\right. }}
\newcommand{\CCDFarray}[3]{{ \left\{\begin{array}{ll}
   1,    & {#3} < {#2} \\
   {#1}, & {#3} \ge {#2} \end{array}\right. }}
\newcommand{\Vector}[1]{\left[ \begin{array}{c} #1 \end{array} \right]}
\newcommand{\PP}[0]{\vspace{0.11in}\noindent}
\newcommand{\Fourier}[1]{{\mathfrak{F}\left\{ {#1}\right\}} }
\newcommand{\IFourier}[1]{{\mathfrak{F}^{-1}\left\{ {#1}\right\}} }
\newcommand{\Laplace}[1]{{\mathfrak{L}\left\{ {#1}\right\}} }
\newcommand{\ILaplace}[1]{{\mathfrak{L}^{-1}\left\{ {#1}\right\}} }
\newcommand{\DTFT}[1]{{\mathrm{DTFT}\left\{ {#1}\right\}} }
\newcommand{\IDTFT}[1]{{\mathrm{DTFT}^{-1}\left\{ {#1}\right\}} }
\newcommand{\rect}[0]{\mbox{rect}}
\newcommand{\sinc}[0]{\mbox{sinc}}
\newcommand{\Sinc}[1]{\frac{\mbox{sin}\left( \pi \left[ {#1} \right] \right)}{\pi \left[ {#1} \right]} }
\newcommand{\SINC}[1]{\frac{\mbox{sin}\left(  {#1} \right)}{ {#1} } }
\newcommand{\Summary}[1]{{\vspace{0.15in} \noindent \bf Summary of today's lecture}: #1\\}
\newcommand{\rank}[0]{\mbox{rank}}
\newcommand{\atantwo}[2]{{\mbox{atan2} \left({#1}, {#2} \right) }}
\newcommand{\erf}[0]{\mbox{erf}}
\newcommand{\erfc}[0]{\mbox{erfc}}
\newcommand{\rightflowbox}[1]{\rightarrow\!\!\boxed{{#1}}\!\!\rightarrow}

\newcommand{\En}[0]{\mathcal{E}}
\newcommand{\Ebno}[0]{\frac{\mathcal{E}_b}{N_0}}
\newcommand{\Question}[0]{{\vspace{0.15in} \noindent \bf Question:  }}
\newcommand{\dB}[1]{{#1}\left[\mbox{dB}\right]}
\newcommand{\dBref}[2]{{#1}\left[\mbox{dB#2}\right]}
\newcommand{\dBm}[1]{{#1}\left[\mbox{dBm}\right]}
\newcommand{\dBW}[1]{{#1}\left[ \mbox{dBW} \right]}
\newcommand{\Span}[1]{\mbox{Span} \{ \mathcal{#1} \}   }
\newcommand{\intinfty}[2]{{\int_{#1 = -\infty}^{\infty} #2  d{#1} }}
\newcommand{\decision}[2]{{{#1 \atop >} \atop {< \atop #2}}}
\newcommand{\Q}[1]{{\mbox{Q}\left( {#1} \right)}}
\newcommand{\Qinv}[1]{{\mbox{Q}^{-1}\left( {#1} \right)}}
\newcommand{\sgn}[1]{{\mbox{sgn}\left\{ {#1} \right\}}}
\newcommand{\entropy}[1]{H\left[ {#1} \right]}
\newcommand{\stdPM}[0]{(P,\mathcal{F}, \Omega)}
\newcommand{\apriori}[0]{\emph{a priori} }
\newcommand{\nnn}[0]{\nonumber \\ }
\newcommand{\nn}[0]{\nonumber }
\newcommand{\sifi}[0]{$\sigma$-field}
\newcommand{\communicateswith}[0]{{\leftrightarrow }}
\newcommand{\MatTwoCols}[1]{\left[ \begin{array}{cc} #1 \end{array} \right]}
\newcommand{\MatThreeCols}[1]{\left[ \begin{array}{ccc} #1 \end{array} \right]}
\newcommand{\MatFourCols}[1]{\left[ \begin{array}{cccc} #1 \end{array} \right]}
\newcommand{\MatFiveCols}[1]{\left[ \begin{array}{ccccc} #1 \end{array} \right]}
\newcommand{\MatSixCols}[1]{\left[ \begin{array}{cccccc} #1 \end{array} \right]}
\newcommand{\MatSevenCols}[1]{\left[ \begin{array}{ccccccc} #1 \end{array} \right]}
\newcommand{\MatEightCols}[1]{\left[ \begin{array}{cccccccc} #1 \end{array} \right]}
\newcommand{\MatNineCols}[1]{\left[ \begin{array}{ccccccccc} #1 \end{array} \right]}
\newcommand{\MatTenCols}[1]{\left[ \begin{array}{cccccccccc} #1 \end{array} \right]}
\newcommand{\MatElevenCols}[1]{\left[ \begin{array}{ccccccccccc} #1 \end{array} \right]}
\newcommand{\limin}[1]{\lim_{{#1}\rightarrow \infty}}
\newcommand{\ep}[1]{{\times 10^{{#1}}}}
\newcommand{\logten}[0]{{\log_{10}}}
\newcommand{\arrowunder}[1]{\mathop{\rightarrow}^{#1}}
\newcommand{\Combinations}[2]{\left( \begin{array}{c} {#1} \\ {#2} \end{array} \right)}
\newcommand{\PRgiven}[2]{P\left[{#1} \, | \, {#2} \right]}

\newcommand{\ThisSemester}[0]{Spring 2022}

